Generalized Disparate Impact for Configurable Fairness Solutions in ML

We make two contributions in the field of AI fairness over continuous protected attributes. First, we show that the Hirschfeld-Gebelein-Renyi (HGR) indicator (the only one currently available for such a case) is valuable but subject to a few crucial limitations regarding semantics, interpretability, and robustness. Second, we introduce a family of indicators that are: 1) complementary to HGR in terms of semantics; 2) fully interpretable and transparent; 3) robust over finite samples; 4) configurable to suit specific applications. Our approach also allows us to define fine-grained constraints to permit certain types of dependence and forbid others selectively. By expanding the available options for continuous protected attributes, our approach represents a significant contribution to the area of fair artificial intelligence.

==> src/related.tex <==
\label{sec:related} 

Ensuring fairness in machine learning is crucial in domains where automated decisions have an impact on people’s lives, like in health, credit, and justice systems. Machine learning models may learn biases from historical data and encode discriminatory behaviors that are endemic in society (e.g., biased recidivism risk \cite{propublica2016}). In many scenarios, designing the model to ignore all the protected attributes is not sufficient to achieve fairness since other features might act as proxies for the protected attributes \cite{Pedreschi2008}.
Thus, as the use of machine learning increases in sensitive domains, there is now a growing interest in defining models that satisfy fairness requirements while preserving high performances. In the following section, we describe several approaches with no intention of offering a comprehensive list. A more extensive review can be found in \cite{10.1145/3457607}.\\


\textbf{Pre-processing and post-processing techniques.} Pre-processing techniques focus on transforming the data in order to mitigate discrimination before training the model. In particular, \cite{DBLP:journals/kais/KamiranC11} investigates different techniques to pre-process the data such as suppressing of the sensitive attribute, changing class labels, and re-sampling the data to remove discrimination. Calmon et al. \cite{NIPS2017_9a49a25d} proposes to reduce discrimination while preserving utility by performing a data transformation learned through a convex optimization.
A different class of techniques for removing discrimination is to calibrate the predictive model once trained. For example, \cite{Calders2010} proposes to adjust the probability learned by the classifier, while \cite{NIPS2016_9d268236} focuses on post-calibrating the classification threshold through a loss minimization. However, all these approaches are deeply linked to the discrete nature of the protected attributes, while \ourmodel applies also to continuous variables.\\

\textbf{In-processing techniques.} The third type of approaches,
which most closely relates to our work, focuses on removing discrimination at learning time. To this goal, \cite{pmlr-v81-menon18a} modify the class-probability estimates during the training, while \cite{10.1007/978-3-642-33486-3_3,Zafar_2017,10.5555/3327144.3327203,ijcai2020p315,pmlr-v80-komiyama18a} embed fairness in the learning procedure through a constraint in the objective. Two recent works \cite{pmlr-v97-mary19a,ijcai2020p313}, extend the method proposed by \cite{6137441} to continuous variables by minimizing the Hirschfeld-Gebelein-Renyi (HGR) correlation coefficient \cite{Rnyi1959OnMO}. 



==> tables/continuous_fine.tex <==
\begin{table*}
\centering
\caption{Performance tests results on the \ourmodel{}-Fine approach for tasks with \textit{continuous} protected feature.}
\label{table:continuous}
\vspace{2pt}
\scriptsize
\begin{tabular}{lccccl|ccccl}
\toprule
{} & \multicolumn{5}{c|}{\textit{Communities \& Crimes}} & \multicolumn{5}{c}{\textit{Adult}} \\
{} & \multicolumn{2}{c}{R2} & \multicolumn{2}{c}{GeDI-V5 \%} & \multicolumn{1}{c|}{Time} & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{GeDI-V5 \%} & {Time} \\
{} & {train} & {val} & {train} & {val} & \multicolumn{1}{c|}{} & {train} & {val} & {train} & {val} & {} \\
\midrule
\it RF &\it 0.95 $\pm$ 0.00 &\it 0.63 $\pm$ 0.02 &\it 1.70 $\pm$ 0.08 &\it 2.03 $\pm$ 0.59 &\it 5.23 &\it 1.00 $\pm$ 0.00 &\it 0.85 $\pm$ 0.00 &\it 3.40 $\pm$ 0.06 &\it 3.76 $\pm$ 0.18 &\it 2.74 \\
~~+MT & 0.48 $\pm$ 0.01 & 0.36 $\pm$ 0.02 & 0.24 $\pm$ 0.01 & 0.64 $\pm$ 0.20 & 61.97 &\bf 0.92 $\pm$ 0.00 & 0.78 $\pm$ 0.00 & \textbf{0.20} $\pm$ 0.00 & 1.13 $\pm$ 0.25 &\bf 256.02 \\
\noalign{\vskip -4pt} & & & & & & & & & & \\
\it GB & 0.87 $\pm$ 0.01 &\it 0.63 $\pm$ 0.02 &\it 1.67 $\pm$ 0.10 &\it 2.09 $\pm$ 0.50 &\it 2.52 &\it 0.87 $\pm$ 0.00 &\it 0.86 $\pm$ 0.00 &\it 3.59 $\pm$ 0.06 &\it 3.59 $\pm$ 0.16 &\it 4.14 \\
~~+MT & 0.47 $\pm$ 0.01 & 0.37 $\pm$ 0.02 & 0.23 $\pm$ 0.00 & \textbf{0.55} $\pm$ 0.24 & 30.58 & 0.81 $\pm$ 0.00 & 0.80 $\pm$ 0.01 & 0.65 $\pm$ 0.06 & 0.76 $\pm$ 0.26 & 658.27 \\
\noalign{\vskip -4pt} & & & & & & & & & & \\
\it NN &\it 0.99 $\pm$ 0.01 &\it 0.58 $\pm$ 0.01 &\it 1.79 $\pm$ 0.14 &\it 1.78 $\pm$ 0.35 &\it 7.58 &\it 0.89 $\pm$ 0.00 &\it 0.83 $\pm$ 0.00 &\it 4.09 $\pm$ 0.16 &\it 4.12 $\pm$ 0.21 &\it 306.42 \\
~~+MT &\bf 0.70 $\pm$ 0.03 & 0.32 $\pm$ 0.05 & 0.27 $\pm$ 0.03 & 1.09 $\pm$ 0.67 & 94.14 & 0.80 $\pm$ 0.01 & 0.79 $\pm$ 0.01 & 0.32 $\pm$ 0.08 & \textbf{0.51} $\pm$ 0.29 & 2096.00 \\
~~+SBR & 0.64 $\pm$ 0.03 &\bf 0.43 $\pm$ 0.04 & \textbf{0.18} $\pm$ 0.03 & 0.92 $\pm$ 0.47 &\bf 15.87 & 0.84 $\pm$ 0.00 &\bf 0.83 $\pm$ 0.00 & 0.89 $\pm$ 0.04 & 0.91 $\pm$ 0.10 & 793.28 \\

\bottomrule
\end{tabular}
\end{table*}

